Patient Specific Biomechanics Are Clinically Significant In Accurate Computer Aided Surgical Image Guidance

Augmented Reality is used in Image Guided surgery (AR IG) to fuse surgical landmarks from preoperative images into a video overlay. Physical simulation is essential to maintaining accurate position of the landmarks as surgery progresses and ensuring patient safety by avoiding accidental damage to vessels etc. In liver procedures, AR IG simulation accuracy is hampered by an inability to model stiffness variations unique to the patients disease. We introduce a novel method to account for patient specific stiffness variation based on Magnetic Resonance Elastography (MRE) data. To the best of our knowledge we are the first to demonstrate the use of in-vivo biomechanical data for AR IG landmark placement. In this early work, a comparative evaluation of our MRE data driven simulation and the traditional method shows clinically significant differences in accuracy during landmark placement and motivates further animal model trials.

==> texsrc/relatedwork.tex <==
\section{Background And Motivation}\label{sec:relatedwork}

%TODO Start off by explaining Figure 1 here say this is how things work and here is the problem we are focused on and what the state of the art is in dealing with it
%Use this section to show that we are adding something to a state of the art framework
%can use that to discuss figure 1
%Background is the SOFA framework motivation is that it is not accurate enough and we can andd a tiny thing to help with that
 
AR IG Frameworks such as SOFA have shown promise in liver procedures but accurate image guidance is challenging. Guidance landmarks within the liver are tracked using a physical simulation. State of the art simulators do not account for patient specific biomechanics, potentially impacting accuracy. This motivates using Magnetic Resonance Elastography scan data in AR IG simulation since the scans measure liver biomechanics.

\subsection{Augmented Reality Image Guidance}

AR IG is implemented using several computer vision algorithms to map preoperative images of liver to a video feed of surgery in progress. Fig~\ref{tab:concept} illustrates the major steps of a canonical AR IG pipeline for a stereo laparoscopic liver procedure. Firstly, the two dimensional laparoscope video feed is mapped to a 3D coordinate system with a 3D reconstruction step. Secondly, change in liver appearance from the previous video frame is tracked using a registration step. Thirdly, an inverse kinematics step computes the force responsible for change in liver appearance. Next, change of the liver appearance visible in the video is propagated to the interior of the liver a with a physical simulation of the force.
Finally, image guidance landmarks are overlaid on the video feed using a coordinate transform step.
We focus on the physical simulation step (gray region of~\cref{tab:concept}) in this work.
Although other pipeline configurations exist for different camera and video monitor configurations, a physical simulation stage is required to accurately place surgical landmarks outside of the camera's field of view. 
Typically the pipeline is modular and constructed using a framework, such as SOFA, meaning advances in one stage can be integrated into a complete system with little effort.

\subsection{Physically Based Surgical Image Guidance}

Real time physical simulation has shown promise in positioning image guidance landmarks during liver procedures although challenges remain~\cite{marques2015framework,haouchine2014towards,pessaux2015towards}. The liver poses many difficulties to real time physical simulation. It is an organ of soft, hyperelastic, and heterogeneous materials that is difficult to model in real time. Researchers are  particularly interested in computationally efficient approximate liver models since AR IG requires video rate simulation. Various approaches to the simulation problem have been tried that make different trade offs. 

Zhang's survey provides a broad overview of surgically oriented simulation approaches that reviews both common and exotic models for real time simulation in surgery~\cite{zhang2018deformable}. To summarize, most research effort has been invested into advanced Finite Element Analysis (FEA) methods that mitigate the issues of large displacements that occur in tissue during surgery~\cite{jia2018cpu,paulus2015surgical,paulus2015augmented}. 
Because of the complexity of surgical scenes, models and simulations are typically packaged in frameworks of simulation libraries which are then configured to perform image guidance. Frameworks include the mass spring SPRING~\cite{montgomery2002spring}
framework, SOFA~\cite{allard2007sofa} which has a modular physics simulator and Nvidia FleX, which uses position based dynamics~\cite{camara2016soft}. Of these frameworks, SOFA is the most mature and feature rich. 

With the improvement in simulator capability, effort has been invested into creating patient specific simulations for accurate image guidance. An advanced approach is described in Haouchine's work which considers heterogeneity of tissue mechanics and anisotropic materials within the liver \cite{haouchine2015impact}. However it focuses mainly on geometry and makes assumptions on model stiffness coefficients from an atlas. Plantefeve's recent work represents the current state of the art in patient specific liver modeling and uses offline segmentation approaches to create separate models of liver blood vessels and parenchyma~\cite{plantefeve2016patient}. Plantefeve mitigates the unrepresentative nature of atlas stiffness data by attempting to modify the elastic modulus of the model to reach convergence with the simulation and video feed online. However the issue with this approach is that the convergence does not take into account heterogeneity of the parenchyma stiffness and modifying the the modulus may yield only superficially better results as much of the liver is out of view during calibration. 

Ideally patient specific image guidance simulation would use a data-driven measurement of the elastic modulus combined with a simulation framework amenable to topology changes caused by cutting. To the best of our knowledge, no image guidance simulator has implemented such a framework because of the difficulty in measuring elastic modulus ($\mathbf{E}$) in vivo. 
However, MRE is a recently developed imaging technique that can measure $\mathbf{E}$ simultaneously as MRI are scanned for constructing the sophisticated models mentioned earlier. 
Although there has been recent investigation into the accuracy of MRE enriched physical simulation~\cite{hollis2016computational}, this work focuses on validation of MRE methodologies. To the best of our knowledge, no work has applied MRE data to the AR IG simulation step.



\subsection{Magnetic Resonance Elastography}
MRE is a non-invasive magnetic resonance imaging method of measuring mechanical properties of tissue in vivo that was first reported by Muthupillai et al. in 1995~\cite{muthupillai1995magnetic}. Its primary clinical use in the liver is as an alternative to biopsy since liver stiffness can be used to evaluate cirrhosis in chronic liver disease~\cite{venkatesh2013magnetic}.

The operating principle of MRE is to induce and detect a shear wave in tissue using a mechanical driver. A acoustic driver is coupled to a non-ferromagnetic diaphragm placed on a patient inside a MRI machine. A series of gradient sensitized MRI are taken while the driver forces a shear wave in the patients tissue. A 2D or 3D elastic modulus map can then be recovered by performing direct wave inversion or other approaches such as local frequency estimation, algebraic inversion of the differential equation, or data-driven hybrid techniques including numerical optimization and machine learning approaches~\cite{manduca2001magnetic,chatelin2016automatic,murphy2018artificial}

MRE research has a strong focus on refining inversion algorithms as it is challenging to recover the elastic modulus. However, despite this, several repeatability studies have shown MRE is an accurate technique for measuring stiffness~\cite{xanthakos2014use,shi2014short,zhang2016short,yasar2016interplatform,hines2010repeatability,venkatesh2014magnetic}. MRE is therefore a promising candidate to enhance simulation accuracy by replacing estimated $\mathbf{E}$ values. 
MRE data is especially interesting for image guidance simulation since patient specific MRE models require zero additional computational overhead and are therefore efficient for real time simulation.
